The Exact Renormalization Group -- renormalization theory revisited --

We overview the entire renormalization theory, both perturbative and non-perturbative, by the method of the exact renormalization group (ERG). We emphasize particularly on the perturbative application of the ERG to the phi4 theory and QED in the four dimensional euclidean space.

==> dining.tex <==
7(F): dinner at Konak (shishi kebap)
8(Sat): lunch at
	dinner at
9(S): lunch at Tuetish
	dinner at 
10(M): dinner at 
11(Tue): dinner at

